Plenoxels: Radiance Fields without Neural Networks

We introduce Plenoxels (plenoptic voxels), a system for photorealistic view synthesis. Plenoxels represent a scene as a sparse 3D grid with spherical harmonics. This representation can be optimized from calibrated images via gradient methods and regularization without any neural components. On standard, benchmark tasks, Plenoxels are optimized two orders of magnitude faster than Neural Radiance Fields with no loss in visual quality.

==> figures_tex/bad.tex <==
\newcommand{\badwidth}{0.49\linewidth}

\begin{figure}[h]
  \centering
  \includegraphics[width=\badwidth]{figures/synthetic/ours_512/badchair.png}
  \includegraphics[width=\badwidth]{figures/synthetic/ours_512/badship.png}
  \caption{\textbf{Our worst artifacts.} When using the same parameters on all 8 synthetic scenes, we notice two main artifacts: some missing geometry on the chair and extra geometry underneath the ship. The missing chair piece is difficult to distinguish from the white background, and the bottom of the ship is sparsely supervised. By tuning parameters per-scene we can correct for these artifacts.}
  \label{fig:bad}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
